Motivic Donaldson-Thomas invariants and McKay correspondence

Let $G\subset SL_2(C)\subset SL_3(C)$ be a finite group. We compute motivic Pandharipande-Thomas and Donaldson-Thomas invariants of the crepant resolution $Hilb^G(C^3)$ of $C^3/G$ generalizing results of Gholampour and Jiang who computed numerical DT/PT invariants using localization techniques. Our formulas rely on the computation of motivic Donaldson-Thomas invariants for a special class of quivers with potentials. We show that these motivic Donaldson-Thomas invariants are closely related to the polynomials counting absolutely indecomposable quiver representations over finite fields introduced by Kac. We formulate a conjecture on the positivity of Donaldson-Thomas invariants for a broad class of quivers with potentials. This conjecture, if true, implies the Kac positivity conjecture for arbitrary quivers.

==> command.tex <==
%%%%% my abbreviations %%%%%%
\RequirePackage{amsmath,amsthm,amssymb,xspace}
%\usepackage[mathscr]{eucal}
%\makeatletter\@for\temp:=\list\do{\temp}\makeatother

\def\makedef#1#2{\expandafter\gdef\csname#1\endcsname{#2}}
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}} 				% \dmat\name{commands}
\def\dmata#1#2{\makedef{#1}{\mat{#2}}}	% \dmata{name}{commands}
\def\dmatb#1{\dmat#1} %open {} for \dmat
\def\makelet#1#2{\expandafter\let\csname#1\expandafter\endcsname\csname#2\endcsname}
\def\redefmath#1{\makelet{temp@#1}{#1}\dmata{#1}{\csname temp@#1\endcsname}}

\def\listdo#1#2{\gdef\listproc{#1}\listdox#2,xxx,}%#1-procedure,#2-list
\def\listend{xxx}
\def\listdox#1,{\def\temp{#1}\ifx\temp\listend\relax\else\listproc{#1}\expandafter\listdox\fi}


%%%% Standard structures and Calligraphic letters, Gothic letter %%%%
\def\defbb#1{\dmata{c#1}{\mathbb{#1}}}		% usage \cA
\def\defcal#1{\dmata{l#1}{\mathcal{#1}}}	% usage \lA
\def\deffrak#1{\dmata{g#1}{\mathfrak{#1}}} % usage \ga,\gA
\def\bbcal#1{\defbb{#1}\defcal{#1}\deffrak{#1}}
\listdo\bbcal{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

%%%% Gothic Letters %%%%%
\listdo\deffrak{a,b,c,d,f,h,i,j,k,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\def\g{\mat{\mathfrak{g}}} %\gg and \ggg are standartly reserved for ">>" and ">>>"
\def\gge{\mat{\mathfrak{e}}} %\ge is reserved for ">="
\def\ggl{\mat{\mathfrak{l}}} %\gl is reserved for "gl", \l is stand. reserved

%%%%% Greek letters %%%%%
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\Ga\Gamma
\dmat\de\delta
\dmat\De\Delta
\dmat\eps\varepsilon
\dmat\Eps\lE
\dmat\epsi\epsilon
\dmat\hi\chi
\dmat\kapa\kappa
\dmat\kp\kappa
\dmat\ksi\xi
\dmat\La\Lambda
\dmat\la\lambda
\dmat\Nabla\bigtriangledown
\dmat\Na\Nabla
\dmat\Om\Omega
\dmat\om\omega
\dmat\vi\varphi
\dmat\si\sigma
\dmat\Si\Sigma
\dmat\ze\zeta
\dmat\te\theta
\dmat\Te\Theta
\dmat\Tau{\mathcal{T}}
\listdo\redefmath{eta,xi,mu,nu,Phi,Psi,psi,pi,rho}

%%%% Functions %%%%%
\def\DMO#1#2{\dmat#1{\operatorname{#2}}}  % \DMO\name{commands}
%\def\DMOx{\DeclareMathOperator} % standard
\def\oper#1{\dmata{#1}{\operatorname{#1}}}


%%% F1:Morphisms...
\listdo\oper{Hom,RHom,Ext,End,Aut,Fun,Tor,ext,hom}
\DMO{\lHom}{\lH\mathit{om}}
\DMO{\lEnd}{\lE\mathit{nd}}
\DMO{\lExt}{\lE\mathit{xt}}

%%% F2:cat related
\listdo\oper{Ob,Mor,Arr,im,coim,coker}
\listdo\oper{Id,id,add,ind,pro,Map,Maps,Iso,Isom,Ind,Bun,Loc}
\def\ilim{\varprojlim} %inverse limit
\def\plim{\ilim}
\def\dlim{\varinjlim} %direct limit
\DMO{\Higgs}{Higgs}
\DMO{\Hitch}{Hitch}
\def\Hig{\Higgs}
\def\Hit{\Hitch}
\makeatletter
\@ifpackageloaded{bbm}
{\def\one{\mathbbm{1}}}
{\def\one{\mathbf{1}}}
\makeatother

%%% F3:cat examples
\DMO{\Presh}{Presh}
\dmat\Sch{\mathbf{Sch}}
\dmat\Cat{\mathbf{Cat}}
\dmat\Set{\mathbf{Set}}
\def\Sets{\Set}
\def\Ab{\mat{\mathbf{Ab}}}
\def\Alg{\mat{\mathbf{Alg}}}
\def\Ring{\mat{\mathbf{Ring}}}
\def\Mon{\mat{\mathbf{Mon}}}
\def\Groupoids{\mat{(\mathbf{Groupoids})}}
\def\Gd{\mat{\mathbf{Gd}}}  %Groupoids
\def\Gp{\mat{\mathbf{Gp}}}  %Groups
\def\SS{\mathbf{sSet}}
\def\sset{\mathbf{sSet}}
\def\sSet{\mathbf{sSet}}
\def\sCat{\mathbf{sCat}}
\def\cosimp{{\mat{{\bf\De}\op}}} %cosimplexes
\def\simp{{\mat{\bf\De}}\xspace} %simplexes
\DMO{\Vect}{Vect}

%%% F4:Modules and algebras
\DMO{\coalg}{Coalg}
\DMO{\Rep}{Rep}
\DMO{\Cor}{Cor}
\DMO{\Mod}{Mod}
\DMO{\rad}{rad}
\DMO{\soc}{soc}
\DMO{\ann}{ann}
\DMO{\pd}{pd}
\def\tors{\mat{\rm tors}}

%%% F5:alg geometry
\DMO{\Spec}{Spec}
\DMO{\Specm}{Specm}
\DMO{\Max}{Max}
\DMO{\spec}{Spec}
\DMO{\Proj}{Proj}
\DMO{\supp}{supp}
\DMO{\Coh}{Coh}
\DMO{\coh}{coh}
\DMO{\Qcoh}{QCoh}
\DMO{\QCoh}{QCoh}
\DMO{\Pic}{Pic}
\DMO{\Div}{Div}
\DMO{\ch}{ch}
\DMO{\Hilb}{Hilb}
\DMO{\Fitt}{Fitt}
\DMO{\Quot}{Quot}
\def\Gm{\mat{{\mathbb G}_{\mathrm m}}}
\DMO{\Gras}{Gr}
\DMO{\Grass}{Gr}
\DMO{\Flag}{Flag}
\DMO{\Jac}{Jac}

\DMO{\cone}{cone}
\DMO{\Tw}{Tw}
\DMO{\rank}{rk}
\DMO{\rk}{rk}
\DMO{\codim}{codim}
\DMO{\cov}{cov}
\DMO{\sgn}{sgn}
\DMO{\td}{td}
\listdo\oper{GL,PGL,SL,SO,SU}
\def\gl{\mat{\mathfrak{gl}}}
\def\sl{\mat{\mathfrak{sl}}}
\DMO{\Der}{Der}
\DMO{\der}{Der}
\DMO{\coder}{Coder}
\DMO{\diag}{diag}
\DMO{\HMod}{HMod} %the homotopy category of modules over DGC
\DMO{\ad}{ad}
\DMO{\Ad}{Ad}
\DeclareMathOperator*{\colim}{colim}
\DeclareMathOperator*{\hocolim}{hocolim}
\DeclareMathOperator*{\holim}{holim}
\DMO{\Ho}{Ho}
\def\Ch{\mathbf{Ch}} %chain complexes
%\def\Gr{\mathbf{Gr}} %graded
\DMO\Gr{Gr}

\def\deop{\cosimp}
\DMO{\har}{char}
\DMO{\sk}{sk}
\DMO{\cosk}{cosk}
\DMO{\Gal}{Gal}
\DMO{\tr}{tr}
\DMO{\Tr}{Tr}
\DMO{\Sh}{Sh}
\DMO{\Is}{Is} %Isometries
\DMO{\Hol}{Hol} %Holomorphic automorphisms
\DMO{\Lie}{Lie} %Lie algebra of a group
\DMO{\Res}{Res} %restriction, residue
\DMO{\irr}{irr} %
\DMO\Irr{Irr} %
\DMO{\Exp}{Exp} %
\DMO{\Log}{Log} %
\DMO{\Pow}{Pow}
\DMO{\pow}{pow}
\DMO{\mult}{mult} %
\DMO{\height}{ht} %
\DMO{\wt}{wt}
%\DMO{\moda}{mod}
\oper{mod}
%\def\mod{\operatorname{mod}}
\DMO{\hd}{hd} %homological dimension
\DMO{\face}{face}
\DMO{\Sym}{Sym}
\DMO{\Com}{Com} % operad Com
\DMO{\Eig}{Eig} 
\DMO{\cl}{cl} 
\DMO{\Li}{Li} 
\listdo\oper{Im,Re}
\listdo\oper{Var,Per}
\DMO{\St}{St}

%%%%% symbols %%%%%%
\def\GIT{/\!\!/}
\def\norm#1{\mat{\lVert#1\rVert}}
\def\n#1{\mat{\lvert#1\rvert}}
\def\lrb#1{\left(#1\right)}
\def\dd{\mat{\partial}}
\def\iso{\simeq}
\def\ts{\otimes}
\def\lts{\mat{\stackrel{\bf L}\otimes}}
\def\tl#1{\mat{\tilde{#1}}}
\def\wtl#1{\mat{\widetilde{#1}}}
\def\what#1{\mat{\widehat{#1}}}
\def\conjug#1{\overline{#1}}
\def\sb{\subset}
\def\sbe{\subseteq}
\def\spe{\supseteq}
\def\sp{\supset}
\def\imp{\mat{\Rightarrow}}
\def\iff{\mat{\Leftrightarrow}}
\def\xarr#1{\xrightarrow{#1}}
\def\sd{\rtimes} %semidirect product
\def\xx{\times}
\def\ox{\otimes}
\def\ms{\backslash} %minus set
\def\pt{\mat{\mathbf {pt}}} %point
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{\mbox{(\!(}#1\mbox{)\!)}} %formal Laurent series ((#1))
%\def\pser#1{\Lbrack#1\Rbrack}
%\def\lser#1{\Lparen #1 \Rparen}
\def\llser#1{\llparenthesis #1 \rrparenthesis}
\def\lpoly{\pser}% reverse compatibility
\def\fser{\lser}% reverse compatibility
\def\vac{\mat{\mathbf{1}}}%vacuum vector
\def\partof{\vdash}
\def\half{\mat{\frac12}}
\def\oh{\half} %one half
\def\bop{\bigoplus}
\def\udim{\lb\dim}

%%% sub/superscripts
\def\op{^{\rm op}}
\def\inv{^{-1}}
%\def\dual{{\!\!\:\text{\textasciicaron}}} %requires textcomp
\def\dual{^\vee}
\def\refl{^{\vee\vee}}
%\def\refl{^{\vee\vee}} %was called refl before
\def\red{_{\rm red}}
\def\tw{^{\rm tw}}
\def\et{_{\rm et}}
\def\cond#1#2{\left.#1\right|_{#2}}  %f|_{x=a}
\def\st{{\rm{st}}}
\def\sst{{\rm{sst}}}
\def\orb{{\rm orb}}
%%%% Structures %%%%%%
\newcommand{\qbinom}[2]{\mat{\genfrac{[}{]}{0pt}{}{#1}{#2}}}  %q-binomial coefficient or Gauss polynomial
\def\ang#1{\mat{\left\langle #1\right\rangle}}
\def\angs#1#2{\mat{\left\langle #1 \mid #2\right\rangle}}
\def\set#1{\mat{\{#1\}}}
\def\sets#1#2{\mat{\{#1\mid#2\}}}
\def\vect#1{\mat{({}\begin{smallmatrix}#1\end{smallmatrix}{})}}
\def\smat#1{\mat{\left(\begin{smallmatrix}#1\end{smallmatrix}\right)}}
\def\case#1{\begin{cases}#1\end{cases}}

%%%% Arrows %%%%%
\def\emb{\hookrightarrow}
\def\mto{\mapsto}
\def\arr{\futurelet\test\arrtest}
\def\arrtest{\ifx^\test\let\next\arra\else\let\next\arrb\fi\next}
\def\arra^#1{\xrightarrow{#1}} \def\arrb{\to}

\def\arrowsD{
\def\mto{{\:\vrule height .9ex depth -.2ex width .04em\!\!\!\;\ar}}
\def\ar{{\:\vrule depth -.52ex height .60ex width 0.85em\;\!\!\rhla\,}}
\def\arr{\futurelet\test\arrtest}
\def\arrtest{\ifx^\test\let\next\arra\else\let\next\arrb\fi\next}
\def\arra^##1{\rTo^{##1}} \def\arrb{\ar}
\def\emb{\futurelet\test\embtest}
\def\embtest{\ifx^\test\let\next\emba\else\let\next\embb\fi\next}
\def\emba^##1{\rInto^{##1}} \def\embb{{\:\rthooka\!\!\!\ar}}
\newarrow{Eq}=====
\def\rrarr{\pile{\rTo\\ \rTo}}
\def\lrarr{\pile{\rTo\\ \lTo}}   
\newarrow{ShortTo}{}{}-->
}

\def\arrowsDStandard{
\newarrow{TeXto}----{->}
\newarrow{TeXinto}C---{->}
\newarrow{TeXonto}----{->>}
\newarrow{TeXdashto}{}{dash}{}{dash}{->}
\newarrow{Eq}=====
\def\ar{\rightarrow}
\def\emb{\futurelet\test\embtest}
\def\embtest{\ifx^\test\let\next\emba\else\let\next\embb\fi\next}
\def\emba^##1{\rTeXinto^{##1}} \def\embb{\hookrightarrow}
\def\rrarr{\pile{\rTo\\ \rTo}}
\def\lrarr{\pile{\rTo\\ \lTo}}   
%\def\embb{\rTeXinto}
}

%%%%% Theorems %%%%%%
\def\theorems{
\newcounter{nthr} %auxiliary counter
\numberwithin{nthr}{section}
\let\theHnthr\thenthr
%solves a problem with hyperref, Heiko <oberdiek@ruf.uni-freiburg.de>
%a different solution: option hypertexnames=false in hyperref
\newtheorem{thr}[nthr]{Theorem}
\newtheorem{prp}[nthr]{Proposition}
\newtheorem{lmm}[nthr]{Lemma}
\newtheorem{crl}[nthr]{Corollary}
\newtheorem{clm}[nthr]{Claim}
\newtheorem{conj}{Conjecture}
\newtheorem{rmr}[nthr]{Remark}
\theoremstyle{definition}
\newtheorem{dfn}[nthr]{Definition}
\newtheorem{exm}[nthr]{Example}
\newtheorem{claim}[nthr]{Claim}
\theoremstyle{remark}
%\newtheorem{rmr}[nthr]{Remark}
}

\def\useElsart{
\def\rqed{\hfill{ }\qed}
\newenvironment{proof}[1][PROOF.]{\begin{pf*}{##1}}{\rqed\end{pf*}}
\def\thr{\thm}
\def\prp{\prop}
\def\lmm{\lem}
\def\crl{\cor}
\def\clm{\claim}
%\def\conj}{\conj}
\def\dfn{\defn}
\def\rmr{\rem}
\def\exm{\exmp}}

\def\useSpringer{
\def\thr{\theorem}
\def\prp{\proposition}
\def\lmm{\lemma}
\def\crl{\corollary}
\def\conj{\conjecture}
\def\dfn{\definition}
\def\rmr{\remark}
\def\exm{\example}}

\def\theoremsSpringer{
\newcounter{nthr} %auxiliary counter
\numberwithin{nthr}{section}
\newtheorem{theorem}        [nthr]{Theorem}
\newtheorem{proposition}    [nthr]{Proposition}
\newtheorem{lemma}          [nthr]{Lemma}
\newtheorem{corollary}      [nthr]{Corollary}
\newtheorem{conjecture}     [nthr]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}     [nthr]{Definition}
\newtheorem{remark}         [nthr]{Remark}
\newtheorem{example}        [nthr]{Example}}

\def\theoremsElsevier{
%prop,thm,lem,cor,conj,defn,rem,exmp,claim,note
\newcounter{nthr}
\newtheorem{thm}    [nthr]{Theorem}
\newtheorem{prop}   [nthr]{Proposition}
\newtheorem{lem}    [nthr]{Lemma}
\newtheorem{cor}    [nthr]{Corollary}
\newtheorem{conj}   [nthr]{Conjecture}
\theoremstyle{definition}
\newtheorem{defn}   [nthr]{Definition}
\newtheorem{rem}    [nthr]{Remark}
\newtheorem{exmp}   [nthr]{Example}}


%%%%%%%%%%%%%%%%%%Margin notes \rem{}%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifrem\remtrue
\def\rem#1{\ifrem\marginpar{\raggedright\footnotesize #1}\fi}

%%%% different %%%%%
\def\ainf{\mat{A_\infty}}
\def\mb#1{\mat{\mathbf{#1}}}
\def\br{\linebreak}
\def\lb#1{\mat{\underline{#1}}} %lower bar
\def\ub#1{\mat{\overline{#1}}}  %upper bar
%\def\over#1#2{\mat{\stackrel #2#1}} % #2 over #1
\def\over#1#2{\mat{\substack{#1\\#2}}} % #2 over #1
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
%\def\eq{\equation}\def\endeq{\endequation}
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

%%%%%% Eprints %%%%%%
\def\eprint#1#2{%
%called from a bbl file, #1 - archive name, #2 - preprint id
\expandafter\ifx\csname eprint@#1\endcsname\relax#1:#2%
\else\def\itemID{#2}\csname eprint@#1\endcsname\fi}

\def\defArchive#1#2{%
%#1 - archive name, #2 - code using \itemID for the preprint id
% archive name should be in lower case
\makedef{eprint@#1}{#2}}

\defArchive{arxiv}{\href{http://arXiv.org/abs/\itemID}{{\tt arXiv:\itemID}}}
\defArchive{numdam}{\href{http://www.numdam.org/item?id=\itemID}{Numdam:\itemID}}

\endinput

%%%%%% EPRINT code for bst files%%%%%%
strings{del str first}
integers{length n}
function{splitter}{
	'del := % delimiter
	'str := % string
	"" 'first :=
	str text.length$ 'length :=
	#1 'n :=
	{n length #1 + <}{
		str n #1 substring$ del = {
			str #1 n #1 - substring$ 'first :=
			str n #1 + length substring$ 'str :=
			length 'n :=
		}{}if$
		n #1 + 'n :=
	}while$
	first str
}

function {format.eprint}{
	eprint empty$ {""}{
		eprint ":" splitter
		swap$ duplicate$ empty$ {
			pop$ "arxiv"
		}{
			"l" change.case$
		}if$
		"\eprint{" swap$ "}{" * * swap$ "}" * *
	}if$
}

%%%%%%% simplified version, only for arXiv %%%%%%%%%%
function {format.eprint}{
	eprint empty$ {""}{
		eprint ":" splitter
		swap$ pop$ 'str :=
		"\href{http://arxiv.org/abs/" str * "}" * 
		"{{\ttfamily arXiv:" * str * "}}" *
	}if$
}
%%%%%% end of EPRINT code %%%%%

